Conformal Certification of Reasoning Trace Prefixes

Language model reasoning traces are rarely all-or-nothing; they frequently contain valid intermediate steps before a critical error occurs. Existing uncertainty quantification methods typically certify final answers or entire responses, failing to provide statistical guarantees for the proportion of a sequential trace that can be safely retained. To address this, we introduce CROP (Conformal Reasoning Output Prefixes), a verifier-agnostic calibration procedure for clean-prefix certification. Given any step-level risk proxy, CROP selects a calibrated threshold and returns the longest contiguous prefix whose step risk proxies remain below it, routing the uncertified suffix for downstream review or repair. Assuming exchangeability, CROP rigorously controls the marginal probability that the returned prefix contains an annotated error. Across six process-labeled reasoning datasets, we demonstrate that standard step-level metrics such as AUROC do not fully capture prefix utility, suggesting verifiers should instead be evaluated by certified prefix length. Furthermore, CROP balances over- and under-withholding and improves downstream repair accuracy by preserving valid intermediate reasoning while discarding misleading suffixes. Ultimately, this work positions prefix certification as a rigorous, practical bridge between process supervision, abstention, and repair. Code available at https://github.com/matthewyccheung/crop.

==> tables/alpha_boundary_sensitivity.tex <==
\begin{table}[t]
\centering
\caption{Boundary sensitivity to the target prefix-contamination risk. Values are mean percentages over 20 trace-level splits; intervals are 95\% normal confidence intervals across splits.}
\label{tab:alpha_boundary_sensitivity}
\small
\begin{tabular}{llrrrrr}
\toprule
Dataset & $\alpha$ & Prefix risk & Prefix kept & Over-withhold & Unsafe overshoot & Boundary dev. \\
\midrule
Arithmetic & 0.025 & 2.0 $\pm$ 0.4 & 93.9 $\pm$ 0.9 & 3.1 $\pm$ 0.8 & 0.9 $\pm$ 0.2 & 3.9 $\pm$ 0.8 \\
 & 0.050 & 4.3 $\pm$ 0.4 & 97.2 $\pm$ 0.4 & 0.6 $\pm$ 0.2 & 1.7 $\pm$ 0.2 & 2.3 $\pm$ 0.3 \\
 & 0.100 & 8.3 $\pm$ 0.0 & 100.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 3.9 $\pm$ 0.1 & 3.9 $\pm$ 0.1 \\
\addlinespace
GSM8K & 0.025 & 2.2 $\pm$ 0.7 & 54.2 $\pm$ 7.5 & 35.4 $\pm$ 7.3 & 1.0 $\pm$ 0.3 & 36.4 $\pm$ 7.1 \\
 & 0.050 & 5.1 $\pm$ 0.8 & 81.6 $\pm$ 4.3 & 9.4 $\pm$ 4.2 & 2.3 $\pm$ 0.4 & 11.7 $\pm$ 4.0 \\
 & 0.100 & 9.2 $\pm$ 0.8 & 90.2 $\pm$ 0.7 & 2.8 $\pm$ 0.5 & 4.3 $\pm$ 0.4 & 7.1 $\pm$ 0.4 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_cpcc_vs_abstention.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\caption{\textbf{CROP exposes partial reasoning that whole-trace abstention
cannot.} Results include Arithmetic and GSM8K only; Boolean is excluded before
the trace-level splits. Each interface is separately calibrated on the pooled
Arithmetic and GSM8K calibration traces. At target risk $\alpha=0.05$, whole-trace abstention
either retains or rejects the full trace, whereas CROP returns a calibrated
prefix. \emph{Kept} is the percentage of original steps retained, and
\emph{Full accept} is the percentage of traces retained in full. Values are
means $\pm 1.96$ standard errors across 20 repeated splits. Bold indicates a
higher retained-step mean within each score source; the paired retention
interval excludes zero only for the PRM-backed scores.}
\label{tab:cpcc_vs_abstention}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}llccc@{}}
\toprule
Score & Object & Emp. risk & Kept & Full accept \\
\midrule
\multirow{2}{*}{Token/format}
& Whole & $4.8\pm0.5$ & $59.8\pm2.7$ & $62.0\pm2.4$ \\
& CROP  & $4.7\pm0.5$ & $\mathbf{60.5\pm2.3}$ & $4.7\pm2.8$ \\
\addlinespace[2pt]
\multirow{2}{*}{Direct PRM}
& Whole & $4.4\pm0.5$ & $85.6\pm1.0$ & $86.5\pm0.9$ \\
& CROP  & $4.4\pm0.4$ & $\mathbf{89.8\pm0.6}$ & $83.7\pm0.8$ \\
\addlinespace[2pt]
\multirow{2}{*}{Trace + PRM}
& Whole & $4.5\pm0.4$ & $86.4\pm1.0$ & $87.4\pm0.9$ \\
& CROP  & $4.6\pm0.4$ & $\mathbf{89.9\pm0.6}$ & $82.2\pm1.3$ \\
\bottomrule
\end{tabular*}
\end{table}

